Faster high-accuracy log-concave sampling via algorithmic warm starts

Understanding the complexity of sampling from a strongly log-concave and log-smooth distribution $\pi$ on $\mathbb{R}^d$ to high accuracy is a fundamental problem, both from a practical and theoretical standpoint. In practice, high-accuracy samplers such as the classical Metropolis-adjusted Langevin algorithm (MALA) remain the de facto gold standard; and in theory, via the proximal sampler reduction, it is understood that such samplers are key for sampling even beyond log-concavity (in particular, for distributions satisfying isoperimetric assumptions). In this work, we improve the dimension dependence of this sampling problem to $\tilde{O}(d^{1/2})$, whereas the previous best result for MALA was $\tilde{O}(d)$. This closes the long line of work on the complexity of MALA, and moreover leads to state-of-the-art guarantees for high-accuracy sampling under strong log-concavity and beyond (thanks to the aforementioned reduction). Our starting point is that the complexity of MALA improves to $\tilde{O}(d^{1/2})$, but only under a warm start (an initialization with constant R\'enyi divergence w.r.t. $\pi$). Previous algorithms took much longer to find a warm start than to use it, and closing this gap has remained an important open problem in the field. Our main technical contribution settles this problem by establishing the first $\tilde{O}(d^{1/2})$ R\'enyi mixing rates for the discretized underdamped Langevin diffusion. For this, we develop new differential-privacy-inspired techniques based on R\'enyi divergences with Orlicz--Wasserstein shifts, which allow us to sidestep longstanding challenges for proving fast convergence of hypocoercive differential equations.

==> sections/lmc_regularity.tex <==


\section{Regularization via diffusions}

We improve on the following classical result of~\citep{bobgenled2001hypercontractivity}.

\begin{theorem}[Previous regularity result]\label{thm:reg-old}
	Suppose that $\nabla^2 V \succeq \alpha  I_d$, where $\alpha \in\R$ (possibly negative), and let ${(\bar P_t)}_{t\ge 0}$ denote the continuous-time Langevin semigroup with stationary distribution $\pi \propto \exp(-V)$. Then
	\begin{align}
		\KL(\mu P_t \mmid \pi)
		&\le \Bigl( \frac{\alpha}{\exp(2\alpha T)-1} \Bigr) \, W_2^2(\mu, \pi)\,.
	\end{align}
\end{theorem}

We build upon the techniques of~\citep{AltTal22mix} to prove the following.

\begin{theorem}[Improved regularity result]~\label{thm:reg-new}
	Suppose that $\alpha I_d \preceq \nabla^2 V \preceq \beta I_d$ for some $-\infty < \alpha \leq \beta < \infty$. (Note that $\alpha$ and $\beta$ may be negative; they are only guaranteed finite.) Then the following holds for any distributions $\mu,\nu \in \cP_2(\R^d)$. 
	\begin{itemize}
		\item \underline{Regularity of discrete-time LMC.} For any number of iterations $N \in \N$ and any stepsize $h > 0$, 
		\begin{align}
			\KL(\mu P_h^N \ \mmid \nu P_h^N)
			\leq
			\left( \frac{1-r^{-2}}{4h(r^{2N}-1)} \right) W_2^2(\mu,\nu)\,,
			\label{eq:reg-new-lmc}
		\end{align}    
		where $r = 1/\max_{\lambda \in \{\alpha,\beta\}} \abs{1 - h \lambda}$.
		\item \underline{Regularity of continuous-time LD.} For any time $T \geq 0$,
		\begin{align}
			\KL(\mu \bar{P}_T \mmid \nu \bar{P}_T )
			\leq 
			\left(\frac{\alpha}{2(\exp(2\alpha T)-1)}  \right) W_2^2(\mu,\nu)\,.
						\label{eq:reg-new-ld}
		\end{align}  
	\end{itemize}
\end{theorem}


Our new regularity result (Theorem~\ref{thm:reg-new}) strictly improves over the previous best regularity result (Theorem~\ref{thm:reg-old}). The improvements are:
\begin{itemize}
	\item Our regularity result improves by a factor of $1/2$. (And is optimal? See Conjecture~\ref{conj:tight}.)
	\item Our regularity result applies to any two measures, and in particular does not require the second measure to be the stationary measure $\pi$.
	\item Our regularity result extends to discretizations of the Langevin diffusion. This is a more general result, because as the discretization timestep $h \to 0$, this discrete-time result recovers the continuous-time result.
\end{itemize}



\begin{conj}[Tightness of Theorem~\ref{thm:reg-new}]\label{conj:tight}
	Consider a continuous-time Langevin semigroup $\{\bar P_t\}_{t \geq 0}$ with stationary distribution $\pi \propto \exp(-V)$. Suppose that for some $\alpha \in \R$, the inequality~\eqref{eq:reg-new-ld} holds for any probability $\mu,\nu \in \cP_2(\R^d)$ and for any time $T \geq 0$. Then $\nabla^2V \succeq \alpha I_d$.
\end{conj}

\subsection{Proof of Theorem~\ref{thm:reg-new}}

We begin by using the biased mixing argument of~\citep{AltTal22mix} based on the PABI technique---albeit with two modifications. The first modification is that  the shift in the shifted KL divergence is performed w.r.t. $W_2$ rather than $W_{\infty}$.\footnote{This use of $W_2$ in PABI will appear soon in forthcoming work [ATW'23]. See also Appendix~\ref{app:deferred} for an alternative proof of the shift-reduction lemma for this $W_2$ shifted KL divergence.} The second modification is that the potential is not necessarily convex (i.e. the eigenvalue bounds $\alpha$ and $\beta$ can be negative). This yields the following. 

\begin{lemma}[Biased mixing]\label{lem:pabi-biased-mixing}
	Consider the setup of Theorem~\ref{thm:reg-new}. Then
	\begin{align*}
		\KL(\mu_N \mmid \nu_N)
		\leq
		\frac{1}{4h}
		\cdot \min_{\substack{a_0, \dots, a_{N-1} \geq 0 \\ \textrm{s.t.} \sum_{n=0}^{N-1} r^{n+1}a_n = W_2(\mu,\nu)}}
		\sum_{n=0}^{N-1} 
		a_n^2\,.
	\end{align*}
\end{lemma}
\begin{proof}
	For shorthand, denote $\mu_n = \mu P_h^n$ and $\nu_n = \nu P_h^n$. Note that a gradient descent step $x \mapsto \phi_h(x) \deq x-h\,\nabla V(x)$ is $1/r$-Lipschitz. Thus
	\begin{align*}
		\KL(\mu_N \mmid \nu_N)
		&= \KL^{(0)}\bigl([{(\phi_h)}_\# \mu_{N-1}] \,Q_{2h} \bigm\Vert [{(\phi_h)}_\# \nu_{N-1}] \,Q_{2h}\bigr) \\
		&\le \KL^{(a_{N-1})}\bigl({(\phi_h)}_\# \mu_{N-1} \bigm\Vert {(\phi_h)}_\# \nu_{N-1}\bigr) + \frac{a_{N-1}^2}{4h} \\
		&\le \KL^{(ra_{N-1})}(\mu_{N-1} \mmid \nu_{N-1}) + \frac{a_{N-1}^2}{4h}\,.
	\end{align*}
	Iterating this, we obtain
	\[
	\KL(\mu_N \mmid \nu_N)
	\leq 
	\KL^{(\sum_{n=0}^{N-1} r^{n+1}a_n)}(\mu \mmid \nu) + \frac{1}{4h} \sum_{n=0}^{N-1}a_n^2\,.
	\]
	The shifted KL vanishes if $(\sum_{n=0}^{N-1} r^{n+1}a_n) = W_2(\mu,\nu)$. The claim follows.
\end{proof}






\begin{proof}[Proof of Theorem~\ref{thm:reg-new}]
	We solve the optimization problem in Lemma~\ref{lem:pabi-biased-mixing} in closed form. This calculation has appeared in a similar form in~\citep[Footnote 11]{AltTal22dp}. The optimal solution is
	\[
	a_n = r^{n-1} \frac{r^2-1}{r^{2N-1}} W_2(\mu,\nu)\,, \qquad\, \forall n < N\,.
	\]
	For our purposes, checking optimality is unnecessary.\footnote{Optimality is not hard to check, and establishes that this is the best possible bound with the PABI techniques, at least in their current form.} Instead, it suffices for our purposes here to just check feasibility. This is clear because $\sum_{n=0}^{N-1} r^{n+1} a_n = W_2(\mu,\nu)$ by plugging in this choice of $\{a_n\}$ and summing a geometric series. Thus, by plugging this solution into Lemma~\ref{lem:pabi-biased-mixing} and simplifying $ \sum_{n=0}^{N-1} 
	a_n^2 = (1 - r^{-2})/(r^{2N}-1) W_2(\mu,\nu)$, we obtain the desired regularity bound for LMC:
	\[
	\KL(\mu P_h^N \mmid \nu P_h^N)
	\leq
	\frac{1}{4h} 
	\cdot \frac{1-r^{-2}}{r^{2N}-1} \cdot W_2^2(\mu,\nu)\,.
	\]
	\par Next, to establish regularity of the continuous-time Langevin Diffusion, we simply take the limit of this regularity result for discrete-time LMC. Specifically, we fix the total elapsed continuous time $T = Nh$, and take the limit as the number of LMC iterations $N \to \infty$. Then since the stepsize $h = T/N \to 0$, the LMC kernel $P_h^N$ converges weakly to the Langevin Diffusion kernel $\bar{P}_T$, and also $r = 1/\max_{\lambda \in \{\alpha,\beta\}} \abs{1 - h\lambda} = 1/(1 - \alpha h)$ for all sufficiently small $h$. Thus
	\begin{align*}
		\KL(\mu \bar{P}_T \mmid \nu \bar{P}_T)
		&\leq
		\lim_{h \to 0}
		\frac{1}{4h}
		\cdot 
		\frac{1-r^{-2}}{r^{2T/h}-1} \cdot W_2^2(\mu,\nu)
		\\ &=
		\lim_{h \to 0}
		\frac{1-(1-\alpha h)^2}{4h ((1 - \alpha h)^{-2 T/h}-1)} W_2^2(\mu,\nu)
		\\ &=
		\frac{\alpha}{2(\exp(2\alpha T)-1)} W_2^2(\mu,\nu)\,.
	\end{align*}
\end{proof}


